The HepMC3 Event Record Library for Monte Carlo Event Generators

In high-energy physics, Monte Carlo event generators (MCEGs) are used to simulate the interactions of high energy particles. MCEG event records store the information on the simulated particles and their relationships, and thus reflects the simulated evolution of physics phenomena in each collision event. We present the HepMC3 library, a next-generation framework for MCEG event record encoding and manipulation, which builds on the functionality of its widely-used predecessors to enable more sophisticated algorithms for event-record analysis. By comparison to previous versions, the event record structure has been simplified, while adding the possibility to encode arbitrary information. The I/O functionality has been extended to support common input and output formats of various HEP MCEGs, including formats used in Fortran MCEGs, the formats established by the HepMC2 library, and binary formats such as ROOT; custom input or output handlers may also be used. HepMC3 is already supported by popular modern MCEGs and can replace the older HepMC versions in many others.

==> HM3-fig.tex <==
\newcommand{\figsize}{
\begin{figure}\centering
\adjustbox{width=1.0\linewidth, height=0.82\linewidth}{
\begin{tikzpicture}
\pgfplotstableread[col sep=space]{./labels.txt}{\loadedtable}
\begin{axis}
[
width=2.5\textwidth,
xmin=-1, xmax=250,
ymin=0.2, ymax=0.55,
xlabel={},ylabel={Size/IO\_GenEvent file size},
 xticklabels from table={\loadedtable}{[index]1},
 xtick=data,
 x tick label style={rotate=90, anchor=east, align=center, font=\bf\Large}, y tick label style={ font=\bf\Large},
      grid=both,
      ylabel style={font=\bf\Huge, yshift=0.2cm},xlabel style={font=\bf\Huge},
     grid style={line width=.1pt, draw=gray!10},
    major grid style={line width=.2pt,draw=gray!50},
     legend style={font={\bf\LARGE}}
 ]
\addplot [mark=o,mark size=3.5pt,color=black, each nth point=4] table [x index=0, y expr={0.5*\thisrowno{3}/\thisrowno{2}}, col sep=space]{./size.txt};
\addlegendentry{Asciiv3$\times 0.5$}
\addplot [mark=x,mark size=3.5pt,color=black, each nth point=4] table [x index=0, y expr={1.0*\thisrowno{4}/\thisrowno{2}}, col sep=space]{./size.txt};
\addlegendentry{IO\_GenEvent+gz}
\addplot [mark=square,mark size=3.5pt,color=red, each nth point=4] table [x index=0, y expr={1.0*\thisrowno{5}/\thisrowno{2}}, col sep=space]{./size.txt};
\addlegendentry{ROOT}
\addplot [mark=triangle,mark size=3.5pt,color=red, each nth point=4] table [x index=0, y expr={1.0*\thisrowno{6}/\thisrowno{2}}, col sep=space]{./size.txt};
\addlegendentry{ROOT TTree}
\end{axis}
\end{tikzpicture}
}
\caption{A graphical}
\label{fig:corralt}
\end{figure}
}


\newcommand{\figtotaltime}{

\begin{figure}\centering
\adjustbox{width=1.0\linewidth, height=0.82\linewidth}{
\begin{tikzpicture}
\pgfplotstableread[col sep=space]{./labels.txt}{\loadedtable}
\begin{axis}
[
width=2.5\textwidth,
xmin=-1, xmax=250,
ymin=0.1, ymax=1.8,
xlabel={},ylabel={Read time/Read time in HepMC2},
 xticklabels from table={\loadedtable}{[index]1},
 xtick=data,
 x tick label style={rotate=90, anchor=east, align=center, font=\bf\Large}, y tick label style={ font=\bf\Large},
      grid=both,
      ylabel style={font=\bf\Huge, yshift=0.2cm},xlabel style={font=\bf\Huge},
     grid style={line width=.1pt, draw=gray!10},
    major grid style={line width=.2pt,draw=gray!50},
     legend style={font={\bf\LARGE}}
 ]
\addplot [mark=o,mark size=3.5pt,color=black,domain=0.01:2.0, each nth point=4] table [x index=0, y expr={1.0*\thisrowno{4}/\thisrowno{2}}, col sep=space]{./totaltime.txt};
\addlegendentry{IO\_GenEvent}
\addplot [mark=x,mark size=3.5pt,color=black,domain=0.01:2.0, each nth point=4] table [x index=0, y expr={1.0*\thisrowno{6}/\thisrowno{2}}, col sep=space]{./totaltime.txt};
\addlegendentry{Asciiv3}
\addplot [mark=square,mark size=3.5pt,color=red,domain=0.01:2.0, each nth point=4] table [x index=0, y expr={1.0*\thisrowno{8}/\thisrowno{2}}, col sep=space]{./totaltime.txt};
\addlegendentry{ROOTTree}
\addplot [mark=triangle,mark size=3.5pt,color=red,domain=0.01:2.0, each nth point=4] table [x index=0, y expr={1.0*\thisrowno{10}/\thisrowno{2}}, col sep=space]{./totaltime.txt};
\addlegendentry{IO\_GenEvent+gzip}
\end{axis}
\end{tikzpicture}
}
\caption{graphical representation of statistical correlation matrix  at .}
\label{fig:corralt}
\end{figure}
}


\newcommand{\figtotaltimecorr}{

\begin{figure}\centering
\adjustbox{width=1.0\linewidth, height=0.82\linewidth}{
\begin{tikzpicture}
\pgfplotstableread[col sep=space]{./labels.txt}{\loadedtable}
\begin{axis}
[
width=2.5\textwidth,
xmin=-1, xmax=250,
ymin=0.1, ymax=1.8,
domain=0.01:2.0,
%    ymode=log,
xlabel={},ylabel={Corr. read time/Corr. read time in HepMC2},
 xticklabels from table={\loadedtable}{[index]1},
 xtick=data,
 x tick label style={rotate=90, anchor=east, align=center, font=\bf\Large}, y tick label style={ font=\bf\Large},
      grid=both,
      ylabel style={font=\bf\Huge, yshift=0.2cm},xlabel style={font=\bf\Huge},
     grid style={line width=.1pt, draw=gray!10},
    major grid style={line width=.2pt,draw=gray!50},
     legend style={font={\bf\LARGE}}
 ]
\addplot [mark=o,mark size=3.5pt,color=black,domain=0.01:2.0, each nth point=4] table [x index=0, y expr={1.0*(\thisrowno{4}-\thisrowno{3})/(\thisrowno{2}-\thisrowno{3})}, col sep=space]{./totaltime.txt};
\addlegendentry{IO\_GenEvent}
\addplot [mark=x,mark size=3.5pt,color=black,domain=0.01:2.0, each nth point=4] table [x index=0, y expr={1.0*(\thisrowno{6}-\thisrowno{5})/(\thisrowno{2}-\thisrowno{3})}, col sep=space]{./totaltime.txt};
\addlegendentry{Asciiv3}
\addplot [mark=square,mark size=3.5pt,color=red,domain=0.01:2.0, each nth point=4] table [x index=0, y expr={1.0*(\thisrowno{8}-\thisrowno{7})/(\thisrowno{2}-\thisrowno{3})}, col sep=space]{./totaltime.txt};
\addlegendentry{ROOTTree}
\addplot [mark=triangle,mark size=3.5pt,color=red,domain=0.01:2.0, each nth point=4] table [x index=0, y expr={1.0*(\thisrowno{10}-\thisrowno{9})/(\thisrowno{2}-\thisrowno{3})}, col sep=space]{./totaltime.txt};
\addlegendentry{IO\_GenEvent+gzip}
\end{axis}
\end{tikzpicture}
}
\caption{A graphical representation of statistical correlation matrix  at .}
\label{fig:corralt}
\end{figure}
}

\newcommand{\figpypy}{

\begin{figure}\centering
\adjustbox{width=1.0\linewidth, height=0.82\linewidth}{
\begin{tikzpicture}
\begin{axis}
[
width=2.0\textwidth,
%height=1.2\textwidth,
xmin=-0.25, xmax=5.25,
ymin=0.0, ymax=11.5,
enlarge x limits={abs=0.05},    
    enlarge y limits={abs=0.0001},
xlabel={},ylabel={Corr. run time/Corr. run time with C++ HepMC2},
xticklabels={{$\mathbf{e^+e^-\rightarrow \mu^+\mu^-}$}, {$\mathbf{e^+e^-\rightarrow q\bar{q}}$} ,{$\mathbf{e^-p\rightarrow e^-X}$},  
            {$\mathbf{pp\rightarrow Z(\mu^+\mu^-)X}$}, {$\mathbf{pp\rightarrow Z(q\bar{q})X}$}, {$\mathbf{pp\rightarrow t\bar{t}X}$},
            {LEP-I}, {LEP-I} ,{HERA-II},  {LHC Run 3}, {LHC Run 3}, {LHC Run 3} },
 xtick={-0.1,0.9,1.9,2.9,3.9,4.9,0.1, 1.1,2.1,3.1,4.1,5.1},
x tick label style={rotate=90,anchor=east, align=center, font=\bf\Large, yshift=-0.1cm,xshift=-0.25cm}, y tick label style={ font=\bf\Large},
      major tick length=0,
      ymajorgrids=true,
      ylabel style={font=\bf\LARGE},xlabel style={font=\bf\Huge},
     grid style={line width=.1pt, draw=gray!10},
    major grid style={line width=.2pt,draw=gray!50},
     legend style={font={\bf\LARGE}, xshift=-1cm}
 ]
\addplot [mark=square,mark size=3.5pt,color=black] table [x expr={1.0*(\thisrowno{1}}, y expr={1.0*(1.0*\thisrowno{7}-1.0*\thisrowno{3})/(1.0*\thisrowno{6}-1.0*\thisrowno{2})}, col sep=space]{./pythia8python.txt};
\addlegendentry{C++ HepMC3 3.2.0, Pythia8 8.2.43}
\addplot [mark=x,mark size=3.5pt,color=blue] table [x expr={1.0*(\thisrowno{1}}, y expr={1.0*(1.0*\thisrowno{8}-1.0*\thisrowno{4})/(1.0*\thisrowno{6}-1.0*\thisrowno{2})}, col sep=space]{./pythia8python.txt};
\addlegendentry{Python 3.6.8 HepMC3 3.2.0, Pythia8 8.2.43}
\addplot [mark=triangle,mark size=3.5pt,color=red] table [x expr={1.0*(\thisrowno{1}}, y expr={1.0*(1.0*\thisrowno{9}-1.0*\thisrowno{5})/(1.0*\thisrowno{6}-1.0*\thisrowno{2})}, col sep=space]{./pythia8python.txt};
\addlegendentry{Python 2.7.5 HepMC3 3.2.0, Pythia8 8.2.43}
\end{axis}
\end{tikzpicture}
}
\caption{A graphical representation of statistical correlation matrix  at .}
\label{fig:corralt}
\end{figure}
}

















==> Makefile <==
#ulimit -u 10000
latexfile=HM3
newname?=HM3
STYLE=cpc

LATEX=  pdflatex -halt-on-error -shell-escape -enable-write18
BIBTEX=bibtex



ifeq ($(STYLE),cpc)
	STYLE_SPECIFIC_FILES=$(latexfile)-cpc.tex  elsarticle-num.bst elsarticle.ins elsarticle.cls
endif


ifeq ($(STYLE),jpc)
	STYLE_SPECIFIC_FILES=$(latexfile)-jpc.tex jpconf.cls iopams.sty  jpconf11.clo HM3.bst
endif


all: $(latexfile)-$(STYLE).pdf


tar:  Makefile $(latexfile)-$(STYLE).fls figurelist-$(STYLE).txt $(constanttables) $(tables)    $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex  $(STYLE_SPECIFIC_FILES)
	rm -rf TAR
	mkdir -p TAR
	mkdir -p TAR/Figures
	mkdir -p TAR/Codes
#	mkdir -p TAR/Tables
#	mkdir -p TAR/ConstantTables
	cp Makefile  $(latexfile).bib  $(latexfile).bst   $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex    $(STYLE_SPECIFIC_FILES) TAR
#	cp $(constanttables) TAR/ConstantTables
#	cp $(tables) TAR/Tables
	cp $(codes) TAR/Codes
	for a in $$(cat   figurelist-$(STYLE).txt); do\
		cp $$a TAR/Figures;\
	done	
	sed -i 's@'$(latexfile)-'@'$(newname)-'@g' TAR/*tex	
	sed -i 's@'$(latexfile)\.bib'@'$(newname)\.bib'@g' TAR/*tex	
	sed -i 's@'$(newname)-3'@'$(latexfile)-3'@g' TAR/*tex	
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/Makefile
	sed -i 's@^STYLE.*@STYLE='$(STYLE)'@g' TAR/Makefile
	sed -i '/@artic/achecked={2},'     TAR/*bib	
	sed -i '/@inproceed/achecked={2},' TAR/*bib	
	sed -i '/@phdthesis/achecked={2},' TAR/*bib	

ifeq ($(STYLE),epjc)
	sed -i 's@\[htbp\]@@g' TAR/$(latexfile)-tab.tex
	sed -i 's@c|@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@|c@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@}|@}@g' TAR/$(latexfile)-tab.tex
endif
	mv TAR/$(latexfile).bst TAR/$(newname).bst 
	mv TAR/$(latexfile).bib TAR/$(newname).bib 
ifeq ($(STYLE),jhep)
	rm TAR/$(newname).bst 
endif
ifeq ($(STYLE),cpc)
	rm TAR/$(newname).bst 

endif
	mv TAR/$(latexfile)-$(STYLE).tex TAR/$(newname)-$(STYLE).tex
	mv TAR/$(latexfile)-txt.tex TAR/$(newname)-txt.tex
	mv TAR/$(latexfile)-abs.tex TAR/$(newname)-abs.tex
	mv TAR/$(latexfile)-tab.tex TAR/$(newname)-tab.tex
#	mv TAR/$(latexfile)-val.tex TAR/$(newname)-val.tex
#	mv TAR/$(latexfile)-def.tex TAR/$(newname)-def.tex
	mv TAR/$(latexfile)-fig.tex TAR/$(newname)-fig.tex
ifeq ($(STYLE),arxiv)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
ifeq ($(STYLE),cpc)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
	rm -f TAR/$(newname)-cpc.spl 
endif
ifeq ($(STYLE),jhep)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	cp TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname).bbl
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif

	tar -zcvf   $(newname).tar.gz -C TAR . 
	#rm -rf TAR


figures=

codes=Codes/reader.cc Codes/readerplugin.cc  Codes/search.cc

$(latexfile)-$(STYLE).fls: $(constanttables) $(tables) \
                    $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex   $(STYLE_SPECIFIC_FILES)
		pdflatex -recorder $(latexfile)-$(STYLE).tex
figurelist-$(STYLE).txt:  $(latexfile)-$(STYLE).fls
		cat $(latexfile)-$(STYLE).fls | grep pdf | grep Figures | sed 's@\./@@g' |sort | cut -f2 -d' '| uniq  > figurelist-$(STYLE).txt
tables=
constanttables=


$(latexfile)-$(STYLE).pdf :  $(figures) $(constanttables) $(tables) \
                    $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex\
                     $(latexfile)-fig.tex  $(STYLE_SPECIFIC_FILES)
	
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
ifeq ($(STYLE),epjc)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
ifeq ($(STYLE),arxiv)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)


pdf : $(latexfile)-$(STYLE).pdf

$(latexfile).rws: $(latexfile)-dict.txt
	aspell --lang=en create master ./$(latexfile).rws < ./$(latexfile)-dict.txt

spell: $(latexfile).rws
		for a in $$(ls -1 $(latexfile)-*.tex | grep -v fig | grep -v tab  | grep -v cpc| grep -v jpc ); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		aspell  --add-extra-dicts=./$(latexfile).rws  -t  --add-tex-command="prog p" --add-tex-command="myfile p" --add-tex-command="mybox p"  --add-tex-command="lstinline p" --add-tex-command="author p" --add-tex-command="institute p" --add-tex-command="text p" --add-tex-command="affil  p" --add-tex-command="Refrs p" --dont-tex-check-comments -d en_GB -c $$a ;\
		done

clean :
	rm -f $(latexfile)-papers.tex
	rm -f *.aux
	rm -f *.lof
	rm -f *.out
	rm -f *.lot
	rm -f *.bbl
	rm -f *.l4l
	rm -f *.log
	rm -f *.blg
	rm -f *.ilg
	rm -f *.aux
	rm -f $(latexfile)*.dvi
	rm -f $(latexfile)*.ps
	rm -f $(latexfile)*.pdf
	rm -f *.toc
	rm -f *.idx
	rm -f *.ind
	rm -f *.nav
	rm -f *.snm



